Localized Visual Feature Aggregation via Focus Pooling for Visuomotor Policies

Focusing on spatially localized, control-relevant visual cues has been shown to improve data efficiency in visuomotor policies by reducing the need to model task-irrelevant visual variation. Existing methods often impose this focus through input preprocessing, such as cropping control- or object-centric regions in RGB images or point-clouds. However, it remains underexplored whether such localized features can be exposed directly from commonly used convolutional neural network (CNN) encoded features. In this paper, we show that intermediate CNN features preserve localized visual context for control, but existing pooling methods fail to aggregate it effectively. We introduce FocusPool, an attention pooling module that selectively aggregates intermediate visual features according to their relevance to the robot's current proprioceptive context. The resulting pooled representation captures task-progressive, control-relevant local information and is used directly for policy learning. Across simulation and real-world experiments, FocusPool improves policy success rates over pooling and explicit local focus methods by 36.2% and 41.2%, with training only 5.8% of encoder parameters.

==> figs/real/real_activation.tex <==
% \begin{figure}[h]
%     \centering
%     \begin{subfigure}{0.7\linewidth}
%         \centering
%         \includegraphics[width=1.0\linewidth]{figs/real/activation_coffee_ssm.png}
%         \caption{Spatial Softmax}
%         \label{fig:coffee-activation-spatial-softmax}
%     \end{subfigure}

%     % \vspace{1mm}

%     \begin{subfigure}{0.7\linewidth}
%         \centering
%         \includegraphics[width=1.0\linewidth]{figs/real/activation_coffee_rvt2.png}
%         \caption{RVT-2}
%         \label{fig:coffee-activation-rvt2}
%     \end{subfigure}

%     % \vspace{1mm}

%     \begin{subfigure}{0.7\linewidth}
%         \centering
%         \includegraphics[width=1.0\linewidth]{figs/real/activation_coffee_focuspool.png}
%         \caption{\methodname{}}
%         \label{fig:coffee-activation-focuspool}
%     \end{subfigure}

%     \caption{\textbf{Feature Activation on Coffee Transport.}
%     Visualization of feature activations for Spatial Softmax, RVT-2, and \methodname{} overlaid on the input images.}
%     \label{fig:real-coffee-activation}
% \end{figure}

% \begin{figure}[h]
%     \centering
%     \begin{subfigure}{0.7\linewidth}
%         \centering
%         \includegraphics[width=1.0\linewidth]{figs/real/activation_table_ssm_success.png}
%         \caption{Spatial Softmax}
%         \label{fig:cleanup-activation-spatial-softmax}
%     \end{subfigure}

%     \vspace{1mm}

%     \begin{subfigure}{0.7\linewidth}
%         \centering
%         \includegraphics[width=1.0\linewidth]{figs/real/activation_table_rvt2_fail.png}
%         \caption{RVT-2}
%         \label{fig:cleanup-activation-rvt2}
%     \end{subfigure}

%     \vspace{1mm}

%     \begin{subfigure}{0.7\linewidth}
%         \centering
%         \includegraphics[width=1.0\linewidth]{figs/real/activation_table_focuspool_success.png}
%         \caption{\methodname{}}
%         \label{fig:cleanup-activation-focuspool}
%     \end{subfigure}

%     \caption{\textbf{Feature Activation on Table Cleanup.}
%     Visualization of feature activations for Spatial Softmax, RVT-2, and \methodname{} overlaid on the input images.}
%     \label{fig:real-cleanup-activation}
% \end{figure}

% \begin{figure}[h]
%     \centering
%     \begin{subfigure}{0.7\linewidth}
%         \centering
%         \includegraphics[width=1.0\linewidth]{figs/real/activation_giraffe_ssm.png}
%         \caption{Spatial Softmax}
%         \label{fig:giraffe-activation-spatial-softmax}
%     \end{subfigure}

%     \vspace{1mm}

%     \begin{subfigure}{0.7\linewidth}
%         \centering
%         \includegraphics[width=1.0\linewidth]{figs/real/activation_giraffe_rvt2.png}
%         \caption{RVT-2}
%         \label{fig:giraffe-activation-rvt2}
%     \end{subfigure}

%     \vspace{1mm}

%     \begin{subfigure}{0.7\linewidth}
%         \centering
%         \includegraphics[width=1.0\linewidth]{figs/real/activation_giraffe_focuspool.png}
%         \caption{\methodname{}}
%         \label{fig:giraffe-activation-focuspool}
%     \end{subfigure}

%     \caption{\textbf{Feature Activation on Giraffe Build.}
%     Visualization of feature activations for Spatial Softmax, RVT-2, and \methodname{} overlaid on the input images.}
%     \label{fig:real-giraffe-activation}
% \end{figure}
